The Impact of Noise Correlation and Channel Phase Information on the Data-Rate of the Single-Symbol ML Decodable Distributed STBCs

Very recently, we proposed the row-monomial distributed orthogonal space-time block codes (DOSTBCs) and showed that the row-monomial DOSTBCs achieved approximately twice higher bandwidth efficiency than the repetitionbased cooperative strategy [1]. However, we imposed two limitations on the row-monomial DOSTBCs. The first one was that the associated matrices of the codes must be row-monomial. The other was the assumption that the relays did not have any channel state information (CSI) of the channels from the source to the relays, although this CSI could be readily obtained at the relays without any additional pilot signals or any feedback overhead. In this paper, we first remove the row-monomial limitation; but keep the CSI limitation. In this case, we derive an upper bound of the data-rate of the DOSTBC and it is larger than that of the row-monomial DOSTBCs in [1]. Secondly, we abandon the CSI limitation; but keep the row-monomial limitation. Specifically, we propose the row-monomial DOSTBCs with channel phase information (DOSTBCs-CPI) and derive an upper bound of the data-rate of those codes. The rowmonomial DOSTBCs-CPI have higher data-rate than the DOSTBCs and the row-monomial DOSTBCs. Furthermore, we find the actual row-monomial DOSTBCs-CPI which achieve the upper bound of the data-rate.

==> DOSTBCcsi.tex <==
\section{Distributed Orthogonal Space-Time Block
Codes with Channel Phase Information}\label{sec:DOSTBCcsi}


In this section, we assume that the relays have the CPI. Under
this assumption, we first define the DOSTBCs-CPI. Then we show
that a DOSTBC-CPI must be a generalized orthogonal design, and
hence, its data-rate can not be larger than that of the
generalized orthogonal design, which is $4/5$ as derived in
\cite{wang}. Compared to the generalized orthogonal design,
however, the DOSTBCs-CPI have some unique properties, which make
us conjecture that the upper bound of the data-rate of the
DOSTBC-CPI should be smaller than $4/5$.




The definition of the DOSTBCs-CPI is similar with that of the
DOSTBCs. Specifically, we define the DOSTBCs in the following way.

\vspace{3mm} {\it Definition 2:} A $K\times T$ matrix $\bmX_C$ is
called a Distributed Orthogonal Space-Time Block Code with Channel
Phase Information (DOSTBC-CPI) in variables $s_1,\cdots,s_N$ if it
satisfies D1.1 and the following equality
 \begin{eqnarray}\label{eqn:orthcsi}
    \bmX_C\bmR^{-1}\bmX_C^H &=& |s_1|^2 \bmD_1 +\cdots +|s_N|^2
    \bmD_N,
    \end{eqnarray}
    where $\bmD_n={\mathrm{diag}}[D_{n,1},\cdots,D_{n,K}]$
    and $D_{n,1},\cdots,D_{n,K}$ are non-zero.
\vspace{3mm}

Like the DOSTBCs, the DOSTBCs-CPI are single-symbol ML decodable
as well. By using the technique in \cite{zhihang} and \cite{elia},
we can show that the DOSTBCs-CPI also achieve the full diversity
order. Furthermore, by following the proof of Theorem
\ref{thm:necessary}, it is not hard to see that a DOSTBC-CPI
satisfies the follow equality
\begin{eqnarray}\label{eqn:orthEcsi}
\bmX_C\bmX_C^H&=&|s_1|^2\bmE_1 + \cdots+ |s_N|^2\bmE_N,
\end{eqnarray}
where $\bmE_n = {\mathrm{diag}}[E_{n,1},\cdots,E_{n,K}]$ and
$E_{n,1},\cdots,E_{n,K}$ are strictly positive. From
(\ref{eqn:orthEcsi}), it is immediate to see that a DOSTBC-CPI
must be a generalized orthogonal design defined in \cite{wang}.
Therefore, the associated matrices $\bmA_k$ and $\bmB_k$ of the
DOSTBCs-CPI satisfy the following conditions
\begin{eqnarray}
\bmA_{k_1}\bmA_{k_2}^H +
\bmB_{k_2}^*\bmB_{k_1}^T&=&\delta_{k_1,k_2}{\mathrm{diag}}[E_{1,k_1},\cdots,E_{N,k_1}]\label{eqn:aabb}\\
\bmA_{k_1}\bmB_{k_2}^H + \bmB_{k_2}^*\bmA_{k_1}^T &=& \bmzero \label{eqn:abba}\\
\bmB_{k_1}\bmA_{k_2}^H + \bmA_{k_2}^*\bmB_{k_1}^T &=&
\bmzero\label{eqn:baab}.
\end{eqnarray}
All the analysis of the generalized orthogonal design in
\cite{wang} are valid for the DOSTBCs-CPI. In particular, the
data-rate of the DOSTBC-CPI can not be larger than the upper bound
$4/5$ of the data-rate of the generalized orthogonal.


Actually, the DOSTBCs-CPI have some unique properties other than
(\ref{eqn:aabb})--(\ref{eqn:baab}). For example, we first have the
following theorem.

\begin{thm}\label{thm:XRX}
If a DOSTBC-CPI $\bmX_C$ in variables $s_1,\cdots,s_N$ exists, we
have
\begin{eqnarray}\label{eqn:orthF}
\bmX_C\bmR\bmX_C^H&=&|s_1|^2\bmF_1 + \cdots+ |s_N|^2\bmF_N,
\end{eqnarray}
where $\bmF_n= {\mathrm{diag}}[F_{n,1},\cdots,F_{n,K}]$.


\end{thm}
\begin{proof}
See Appendix C.
\end{proof}

Based on Theorem \ref{thm:XRX}, some properties of the associated
matrices $\bmA_k$ and $\bmB_k$ are obtained and given in the
following lemma.

\begin{lemma}\label{lem:CSIABcond}
If a DOSTBC $\bmX_C$ in variables $s_1,\cdots,s_N$ exists, its
associated matrices $\bmA_k$ and $\bmB_k$, $1\leq k\leq K$,
satisfy the following conditions:
\begin{equation}\label{eqn:CSIcond1}
\bmA_{k_1}(\bmA_i^H\bmA_i +\bmB_i^H\bmB_i)\bmA_{k_2}^H +
\bmB_{k_2}^*(\bmA_i^H\bmA_i +\bmB_i^H\bmB_i)\bmB_{k_1}^T
=\delta_{k_1,k_2}
{\mathrm{diag}}[F_{1,k}^{f_i},\cdots,F_{N,k}^{f_i}]
\end{equation}
\begin{eqnarray}
\bmA_{k_1} (\bmA_i^H\bmA_i +\bmB_i^H\bmB_i) \bmB_{k_2}^H +
\bmB_{k_2}^{*}(\bmA_i^H\bmA_i +\bmB_i^H\bmB_i)
\bmA_{k_1}^T &=& \bmzero\label{eqn:CSIcond2}\\
\bmB_{k_1}(\bmA_i^H\bmA_i +\bmB_i^H\bmB_i)\bmA_{k_2}^H +
\bmA_{k_2}^*(\bmA_i^H\bmA_i +\bmB_i^H\bmB_i)\bmB_{k_1}^T &=&
\bmzero,\label{eqn:CSIcond3}
\end{eqnarray}
where $F_{n,k}^{f_i}$ is a constant and it is decided by
$F_{n,k}=\sum_{i=1}^K F_{n,k}^{f_i} |\rho f_i|^2 + F_{n,k}^{0}$.
\end{lemma}
\begin{proof}
See Appendix D.
\end{proof}


By comparing (\ref{eqn:CSIcond1})--(\ref{eqn:CSIcond3}) with
(\ref{eqn:aabb})--(\ref{eqn:baab}), we see that the DOSTBCs-CPI
have stronger constraints on $\bmA_k$ and $\bmB_k$ than the
generalized orthogonal design. Therefore, we conjecture that the
DOSTBCs-CPI should have an upper bound smaller than $4/5$.
However, it is very hard to derive this upper bound in general.
This is because there is a crucial difference between
(\ref{eqn:CSIcond1}) and (\ref{eqn:aabb}). In (\ref{eqn:aabb}),
the summation always has full rank when $k_1=k_2$ and the
full-rankness plays a key role in the derivation of the upper
bound $4/5$ for the generalized orthogonal design \cite{wang}.
However, the summation in (\ref{eqn:CSIcond1}) may not have full
rank when $k_1=k_2$. This rank deficiency makes it very hard to
derive an upper bound for the DOSTBCs-CPI in general.


The rank deficiency of (\ref{eqn:CSIcond1}) is actually because
the noise covariance matrix $\bmR$ is not diagonal in general. On
the other hand, as we have seen in \cite{zhihang}, constraining
$\bmR$ to be a diagonal matrix can greatly simplify the derivation
of the upper bound of the data-rate. Thus, we restrict our further
interests to some special DOSTBCs-CPI, which generate diagonal
noise covariance matrix at the destination.























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> del_part.tex <==

When $k_1=k_2=k$, the value of $[\bmX\bmR\bmX^H]_{k,k}$ is given
by
\begin{equation}\label{eqn:xrxkk}
[\bmX\bmR\bmX^H]_{k,k}=\sum_{w=1}^W\sum_{t=1}^{T_w}[\bmX_w]_{k,t}
[\bmX_w]_{k,t}^*R_w = \sum_{n=1}^N |s_n|^2F_{n,k}.
\end{equation}
We first notice that the summation of any non-zero terms in
(\ref{eqn:xrxkk}) can not be zero; otherwise, it violates the
row-monomial condition. Therefore, the summation
$\sum_{t=1}^{T_w}[\bmX_w]_{k,t} [\bmX_w]_{k,t}^*R_w$ can be
denoted by
\begin{equation}
\sum_{t=1}^{T_w}[\bmX_w]_{k,t} [\bmX_w]_{k,t}^*R_w = \bms_w^k
\bmG_w^k\bms_w^{kH},
\end{equation}
where $\bms_w^k$ denotes all the symbols transmitted by the $k$-th
row of $\bmX_w$ and it is a subset of $\bms$. The matrices
$\bmG_w^k$ are diagonal and the main diagonal entries are all
non-zero. The values of $\bmG_w^k$ are decided by the following
equation
\begin{equation}
\sum_{w=1}^W \bms_w^k \bmG_w^k\bms_w^{kH}=\sum_{n=1}^N
|s_n|^2F_{n,k}.
\end{equation}
Furthermore, we have already seen that, if one symbol is
transmitted in one row in $\bmX_w$, it must be transmitted by all
other non-zero rows in $\bmX_w$, which implies
$\bms_w^1=\cdots=\bms_w^{K_w}=:\bms_w$. Therefore, we have
$[\bmX_w\bmR_w\bmX_w^H]_{k,k} = \bms_w\bmG_w^k\bms_w^H $. Since we
have already shown that $\sum_{t=1}^{T_w}[\bmX_w]_{k_1,t}
[\bmX_w]_{k_2,t}^*R_w = 0$ for $k_1\neq k_2$, we conclude that
$[\bmX_w\bmR_w\bmX_w^H] = \bms_w{\mathrm{diag}}
[\bmG_w^1,\cdots,\bmG_w^{K_w}] \bms_w^H $, which means $\bmX_w$ is
a row-monomial DOSTBC on symbols $\bms_w$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 we have
\begin{eqnarray}
\bmA_{k_1}(\bmR-\bmI)\bmA_{k_2}^H +
\bmB_{k_2}^*(\bmR-\bmI)\bmB_{k_1}^T &=& \bmzero \label{eqn:a1a2b2b1}\\
\bmA_{k_1} (\bmR-\bmI) \bmB_{k_2}^H + \bmB_{k_2}^{*}(\bmR-\bmI)
\bmA_{k_1}^T &=& \bmzero\label{eqn:a1b2b2a1}\\
\bmB_{k_1}(\bmR-\bmI)\bmA_{k_2}^H +
\bmA_{k_2}^*(\bmR-\bmI)\bmB_{k_1}^T &=&
\bmzero\label{eqn:b1a2a2b1}.
\end{eqnarray}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Consequently, $S={\mathrm{rank}}[\bmA_1;\bmB_1]-N = T-N$. The
uniform transformation in Lemma \ref{lem:CSIABcond} makes
$\overline{\bmA}_1$ and $\overline{\bmB}_1$ have the following
forms \cite{wang}
\begin{eqnarray}
\overline{\bmA}_1 =\left(%
\begin{array}{cccc}
  \bmD_{\lambda} & \bmzero & \bmzero \\
  \bmzero & \bmI & \bmzero \\
\end{array}%
\right)&&
\overline{\bmB}_1 =\left(%
\begin{array}{cccc}
  \bmzero & \bmzero & \bmD_{\mu} \\
  \bmzero & \bmzero & \bmzero \\
\end{array}%
\right).
\end{eqnarray}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Like in Appendix F, we still partition $\bmR$ and $\bmX_C$ into
$\bmR = {\mathrm{diag}}[\bmR_1,\cdots,\bmR_W]$ and $\bmX_C
=[\bmX_{C1},\cdots,\bmX_{Cw}]$, respectively. Let
$\tilde{\bmX}_{Cw}$ denote all the non-zero rows in $\bmX_{Cw}$.
We assume that the dimension of $\tilde{\bmX}_{Cw}$ is $K_w\times
T_w$, and hence, $\sum_{w=1}^W T_w =T$. Furthermore, assume that
$K_1=1$, $K_2=2$, and $K_w>2$ for $3\leq w \leq W$. Let $N_w$
denote the number of different information-bearing symbols
transmitted by $\tilde{\bmX}_{Cw}$. Because one
information-bearing symbol may be transmitted by several different
$\tilde{\bmX}_{Cw}$, $\sum_{w=1}^W N_w \geq N$.


As we have seen, $\tilde{\bmX}_{Cw}$ are row-monomial DOSTBCs.
Furthermore, we have seen in Appendix F that every entry in
$\tilde{\bmX}_{Cw}$ is non-zero. Thus, the full rank constraint in
Theorem \ref{thm:upperDOSTBCcsi} is satisfied. When $3\leq w\leq
W$, the data-rate of $\tilde{\bmX}_{Cw}$ is exactly $1/2$ by
Theorem \ref{thm:upperDOSTBCcsi}. Therefore, we have $\sum_{w=3}^W
T_w \geq 2\sum_{w=3}^W N_w$.\footnote{It is possible that one
information-bearing symbol is transmitted in several different
$\tilde{\bmX}_{Cw}$. In this case, $\sum_{w=3}^W T_w$ will be
strictly larger than $2\sum_{w=3}^W N_w$.} When $w=1$ and $w=2$,
because $\tilde{\bmX}_{Cw}$ can have two rows at most,
$\tilde{\bmX}_{C1}$ and $\tilde{\bmX}_{C2}$ are actually the
row-monomial DOSTBCs defined in \cite{zhihang}, and hence,
$T_1+T_2 \geq 2(N_1+N_2)$ by Theorem 2 in \cite{zhihang}.
Consequently, the data-rate $N/T$ of the row-monomial DOSTBCs is
upper-bounded by
\begin{equation}
\frac{N}{T} \leq \frac{\sum_{w=1}^W N_w}{\sum_{w=1}^W T_w}\leq
\frac{1}{2}.
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Furthermore, let $\overline{\bmA}_k=
\bmW_1\bmA_k\bmV+\bmW_2^*\bmB_k\bmV$ and $\overline{\bmB}_k=
\bmW_2\bmA_k\bmV+\bmW_1^*\bmB_k\bmV$, where $\bmV$ and $\bmU =
[\bmW_1,\bmW_2;\bmW_2^*,\bmW_1^*]$ are unitary matrices. The
matrices $\overline{\bmA}_k$ and $\overline{\bmB}_k$ still satisfy
(\ref{eqn:CSIcond1})--(\ref{eqn:CSIcond3}) and they have the
following forms: when $k=1$,
\begin{eqnarray}\label{eqn:AB1sub}
\overline{\bmA}_1 =\left(%
\begin{array}{cccc}
  \bmD_{\lambda} & \bmzero & \bmzero & \bmzero \\
  \bmzero & \bmI & \bmzero & \bmzero \\
\end{array}%
\right)&&
\overline{\bmB}_1 =\left(%
\begin{array}{cccc}
  \bmzero & \bmzero & \bmD_{\mu} & \bmzero \\
  \bmzero & \bmzero & \bmzero & \bmzero \\
\end{array}
\right);
\end{eqnarray}
when $k>1$,
\begin{eqnarray}\label{eqn:ABksub}
\overline{\bmA}_k =\left(%
\begin{array}{cccc}
  \overline{\bmA}_{k1} & \overline{\bmA}_{k3} & \bmzero & \overline{\bmA}_{k7} \\
  \bmzero & \bmzero & \bmzero & \overline{\bmA}_{k8} \\
\end{array}%
\right)&&
\overline{\bmB}_k =\left(%
\begin{array}{cccc}
  \overline{\bmB}_{k1} & \bmzero & \overline{\bmB}_{k5} & \overline{\bmB}_{k7} \\
  \bmzero & \overline{\bmB}_{k4} & \bmzero & \overline{\bmB}_{k8}
\end{array}%
\right).
\end{eqnarray}


Secondly, we prove (\ref{eqn:ABksub}). By \cite{wang}, the uniform
transform on $\bmA_1$ and $\bmB_1$ can generate
$\overline{\bmA}_1$ and $\overline{\bmB}_1$ as follows:
\begin{eqnarray}
\overline{\bmA}_1 =\left(%
\begin{array}{cccc}
  \bmD_{\lambda} & \bmzero & \bmzero & \bmzero \\
  \bmzero & \bmI & \bmzero & \bmzero \\
\end{array}%
\right)&&
\overline{\bmB}_1 =\left(%
\begin{array}{cccc}
  \bmzero & \bmzero & \bmD_{\mu} & \bmzero \\
  \bmzero & \bmzero & \bmzero & \bmzero \\
\end{array}%
\right),
\end{eqnarray}
where
$\bmD_{\lambda}={\mathrm{diag}}[\lambda_1,\cdots,\lambda_S]$,
$\bmD_{\mu}={\mathrm{diag}}[\mu_1,\cdots,\mu_S]$. Furthermore,
$1>\lambda_k\geq\mu_k>0$ and
$S={\mathrm{Rank}}([\bmA_1;\bmB_1])-N$. When $k>1$, we have
\cite{wang}
\begin{eqnarray}\label{eqn:akbkzero}
\overline{\bmA}_k =\left(%
\begin{array}{cccc}
  \overline{\bmA}_{k1} & \overline{\bmA}_{k3} & \overline{\bmA}_{k5} & \overline{\bmA}_{k7} \\
  \bmzero & \bmzero & \bmzero & \overline{\bmA}_{k8} \\
\end{array}%
\right)&&
\overline{\bmB}_k =\left(%
\begin{array}{cccc}
  \overline{\bmB}_{k1} & \overline{\bmB}_{k3} & \overline{\bmB}_{k5} & \overline{\bmB}_{k7} \\
  \overline{\bmB}_{k2} & \overline{\bmB}_{k4} & \overline{\bmB}_{k6} & \overline{\bmB}_{k8}
\end{array}%
\right).
\end{eqnarray}
The dimensions of the sub-matrices $\overline{\bmA}_{ki}$ and
$\overline{\bmB}_{ki}$ are specified in \cite{wang}, and hence, we
do not repeat them here. Like in \cite{wang}, we can show that the
uniform transform does not change the properties of $\bmA_k$ and
$\bmB_k$, i.e. $\overline{\bmA}_k$ and $\overline{\bmB}_k$ still
satisfy (\ref{eqn:aabb})--(\ref{eqn:baab}) and
(\ref{eqn:CSIcond1})--(\ref{eqn:CSIcond3}).


It follows from (\ref{eqn:aabb}) that
$\overline{\bmA}_{1}\overline{\bmA}_{k}^H+\overline{\bmB}_{k}^*\overline{\bmB}_{1}^T=0$
for $k\neq 1$ and we have
\begin{eqnarray}
\overline{\bmA}_{1}\overline{\bmA}_{k}^H+\overline{\bmB}_{k}^*\overline{\bmB}_{1}^T=\left(%
\begin{array}{cc}
  \bmD_{\lambda}\overline{\bmA}_{k1}^H+\overline{\bmB}_{k5}^*\bmD_{\mu} & \bmzero \\
  \overline{\bmA}_{k3}^H+\overline{\bmB}_{k6}^*\bmD_{\lambda} & \bmzero \\
\end{array}%
\right)=\bmzero,
\end{eqnarray}
which means
$\overline{\bmA}_{k3}^H+\overline{\bmB}_{k6}^*\bmD_{\lambda}=\bmzero$.
On the other hand, by (\ref{eqn:CSIcond1}),
$\overline{\bmA}_{1}(\overline{\bmA}_1^H\overline{\bmA}_1
+\overline{\bmB}_1^H\overline{\bmB}_1)\overline{\bmA}_{k}^H+\overline{\bmB}_{k}^*(\overline{\bmA}_1^H\overline{\bmA}_1
+\overline{\bmB}_1^H\overline{\bmB}_1)\overline{\bmB}_{1}^T=0$ for
$k>1$ and it implies
$\overline{\bmA}_{k3}^H+\overline{\bmB}_{k6}^*\bmD_{\lambda}\bmD_{\lambda}\bmD_{\lambda}=\bmzero$.
Thus,
$\overline{\bmB}_{k6}^*\bmD_{\lambda}\bmD_{\lambda}\bmD_{\lambda}=\overline{\bmB}_{k6}^*\bmD_{\lambda}$.
Because $\bmD_{\lambda}$ is diagonal and $1>\lambda_s$, it is not
hard to see that $\overline{\bmB}_{k6}=\bmzero$ and
$\overline{\bmA}_{k3}=\bmzero$ for $k\neq 1$.



By (\ref{eqn:abba}),
$\overline{\bmA}_1\overline{\bmB}_k^H+\overline{\bmB}_k^*\overline{\bmA}_1^T=\bmzero$
and it implies
$\bmD_{\lambda}\overline{\bmB}_{k2}^H+\overline{\bmB}_{k3}^*=\bmzero$.
Furthermore, by (\ref{eqn:CSIcond2}),
$\overline{\bmA}_1(\bmA_1^H\bmA_1
+\bmB_1^H\bmB_1)\overline{\bmB}_k^H+\overline{\bmB}_k^*(\bmA_1^H\bmA_1
+\bmB_1^H\bmB_1)\overline{\bmA}_1^T=\bmzero$ and it implies
$\bmD_{\lambda}\bmD_{\lambda}\bmD_{\lambda}\overline{\bmB}_{k2}^H+\overline{\bmB}_{k3}^*=\bmzero$.
Because $\bmD_{\mu}$ is diagonal and $1>\mu_s$, it is not hard to
get $\overline{\bmB}_{k2}=\bmzero$ and
$\overline{\bmB}_{k3}=\bmzero$.



Lately, by (\ref{eqn:baab}),
$\overline{\bmB}_1\overline{\bmA}_k^H+\overline{\bmA}_k^*\overline{\bmB}_1^T=\bmzero$
and it implies
$\bmD_{\mu}\overline{\bmA}_{k5}^H+\overline{\bmA}_{k5}^*\bmD_{\mu}=\bmzero$.
On the other hand, by (\ref{eqn:CSIcond3}),
$\overline{\bmB}_1(\bmA_1^H\bmA_1
+\bmB_1^H\bmB_1)\overline{\bmA}_k^H+\overline{\bmA}_k^*(\bmA_1^H\bmA_1
+\bmB_1^H\bmB_1)\overline{\bmB}_1^T=\bmzero$ for $k>1$ and it
leads to
$\bmD_{\mu}\overline{\bmA}_{k5}^H+\overline{\bmA}_{k5}^*\bmD_{\mu}=\bmzero$.
Due to the property of $\bmD_{\mu}$, we obtain
$\overline{\bmA}_{k5}=\bmzero$. Because the sub-matrices
$\overline{\bmB}_{k2}$, $\overline{\bmB}_{k3}$,
$\overline{\bmB}_{k6}$, $\overline{\bmA}_{k3}$, and
$\overline{\bmA}_{k5}$ are all-zero matrices, it is immediate to
obtain (\ref{eqn:ABksub}) from (\ref{eqn:akbkzero}).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

On the other hand, Wang {\it et al.} derived a second upper bound
$K/(2K-2)$ for the generalized orthogonal design in \cite{wang}
under a rank constraint $T =
\max_{k=1,\cdots,K}{\mathrm{Rank}}(\bmA_k;\bmB_k)$. In the
following, we adopt this rank constraint and show that the
data-rate of the DOSTBCs-CPI is exactly $1/2$ when $K>2$.

\begin{thm}\label{thm:upperDOSTBCcsi}
If $K > 2$ and $T =
\max_{k=1,\cdots,K}{\mathrm{Rank}}(\bmA_k;\bmB_k)$, the data-rate
of the DOSTBC-CPI is exactly $1/2$.
\end{thm}
\begin{proof}
See Appendix E.
\end{proof}


The rank constraint $T =
\max_{k=1,\cdots,K}{\mathrm{Rank}}(\bmA_k;\bmB_k)$ actually means
that there is at least one row in $\bmX_C$, whose entries are all
non-zero. We notice that the rate-halving codes developed in
\cite{tarokh} satisfy this rank constraint and they also satisfy
Definition 2. Therefore, the DOSTBCs-CPI achieving the data-rate
$1/2$ are just the rate-halving codes. Without the rank
constraint, we have not found an upper bound of the data-rate of
the DOSTBC-CPI yet. The major hindrance actually comes from the
non-diagonality of $\bmR$. Therefore, we restrict our interests to
a special subset of the DOSTBCs-CPI, whose codes have diagonal
covariance matrices.



\appendices
%\vspace{1cm}
\section*{Appendix E}
\renewcommand\theequation{E.\arabic{equation}}
\setcounter{equation}{0}


Without loss of generality, we assume
$T={\mathrm{rank}}[\bmA_1;\bmB_1]$. It is easy to check that all
the analysis in Appendix D will still hold. Furthermore,
$\overline{\bmA}_{k7}$, $\overline{\bmA}_{k8}$,
$\overline{\bmB}_{k7}$, $\overline{\bmB}_{k8}$ automatically
diminish due to $T={\mathrm{rank}}[\bmA_1;\bmB_1]$ \cite{wang}.
Therefore, when $k>1$, $\overline{\bmA}_k$ and $\overline{\bmB}_k$
are given by
\begin{eqnarray}
\overline{\bmA}_k =\left(%
\begin{array}{cccc}
  \overline{\bmA}_{k1} &\bmzero& \overline{\bmA}_{k5}  \\
  \bmzero & \bmzero & \bmzero \\
\end{array}%
\right)&&
\overline{\bmB}_k =\left(%
\begin{array}{cccc}
  \overline{\bmB}_{k1} & \bmzero & \overline{\bmB}_{k5}  \\
  \bmzero & \overline{\bmB}_{k4} & \bmzero
\end{array}%
\right),
\end{eqnarray}
where the dimension of $\overline{\bmB}_{k4}$ is $(2N-T)\times
(2N-T)$.


Because $\overline{\bmA}_k$ and $\overline{\bmB}_k$ satisfy
(\ref{eqn:aabb}), we first notice that (\ref{eqn:aabb}) becomes
$\overline{\bmA}_{k1}\overline{\bmA}_{k2}^H+\overline{\bmB}_{k2}^*\overline{\bmB}_{k1}^T=\bmzero$
and it implies
$\overline{\bmB}_{k_24}^*\overline{\bmB}_{k_14}^T=\bmzero$, when
$k_1\neq k_2$ and they are both larger than one. When
$k_1=k_2=k>1$, (\ref{eqn:aabb}) becomes
$\overline{\bmA}_{k}\overline{\bmA}_{k}^H+\overline{\bmB}_{k}^*\overline{\bmB}_{k}^T=
{\mathrm{diag}}[E_{1,k},\cdots,E_{N,k}]$ which implies
$\overline{\bmB}_{k4}^*\overline{\bmB}_{k4}^T$ has full rank.
Therefore, the $(2N-T)(K-1)$ rows in the matrix
$[\overline{\bmB}_{24};\overline{\bmB}_{34};\cdots;\overline{\bmB}_{K4}]$
are linearly independent and this leads to $(2N-T)(K-1)\leq 2N-T$.
Because $K>2$, we get $2N-T\leq0$, and hence, $2N\leq T$. On the
other hand, because $T={\mathrm{rank}}[\bmA_1;\bmB_1]$ and the
dimension of $[\bmA_1;\bmB_1]$ is $2N\times T$, we have $T\leq
2N$. Therefore, $T=2N$ and the data-rate $N/T$ is exactly $1/2$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Inspired by \cite{hua}--\cite{jing3}, we think that exploiting the
channel phase information (CPI) at the relays can potentially
increase the data-rate. Therefore, we proposed a new kind of
DSTCs, namely {\it DOSTBC with channel phase information}
(DOSTBC-CPI). Like the DOSTBCs, the DOSTBCs-CPI are single-symbol
ML decodable and achieve the full diversity order. Furthermore, we
show that the data-rate of the the DOSTBC-CPI is upper-bounded by
the data-rate of the generalized orthogonal design, which is $4/5$
as shown in \cite{wang}. Because the DOSTBCs-CPI have some
distinct properties, however, we conjecture that the upper bound
of the data-rate of the DOSTBC-CPI should be smaller than $4/5$,
although it is very hard to derive such upper bound. This is
because the noises at the destination are correlated in general.
Therefore, like in \cite{zhihang}, our further studies are given
to some special DOSTBCs-CPI, which generate uncorrelated noises at
the destination.\footnote{Actually, in most previous publications
about the DSTCs such as \cite{jing1} and \cite{hua}--\cite{jing3},
the authors have mainly considered the codes which generate
uncorrelated noises at the destination.} We refer to those codes
as {\it row-monomial DOSTBCs-CPI} and we derive an upper bound of
the data-rate of the row-monomial DOSTBC-CPI. As we expect, the
row-monomial DOSTBCs-CPI have better bandwidth efficiency than the
DOSTBCs, which is due to the use of the CPI. Furthermore, the
upper bound of the data-rate of the row-monomial DOSTBC-CPI is
independent of the number $K$ of the relays, which ensures the
codes have good bandwidth efficiency even when there are many
relays.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 We
first prove (\ref{eqn:orthE}) by evaluating $[\bmR]_{t_1,t_2}$ and
$[\bmR^{-1}]_{t_1,t_2}$. By (\ref{eqn:R}), when $t_1\neq t_2$,
$[\bmR]_{t_1,t_2}$ can be either null or a sum of several terms
containing $|\rho f_k|^2$; when $t_1 = t_2 = t$, $[\bmR]_{t,t}$ is
a sum of a constant 1, which is from the identity matrix, and
several terms containing $|\rho f_k|^2$. Therefore, we can rewrite
$[\bmR]_{t,t}$ as $[\bmR]_{t,t}=\bar{R}_{t,t}+1$, where
$\bar{R}_{t,t}$ accounts for all the terms containing $|\rho
f_k|^2$. $[\bmR^{-1}]_{t_1,t_2}$ is given by
$[\bmR^{-1}]_{t_1,t_2} = C_{t_2,t_1}/\mathrm{det}(\bmR)$, where
$C_{t_2,t_1}$ is the matrix cofactor of $[\bmR]_{t_2,t_1}$. When
$t_1 =t_2=t$, by the definition of matrix cofactor, $C_{t,t}$
contains a constant 1 generated by the product $\prod_{i=1,i\neq
t}^T [\bmR]_{i,i} = \prod_{i=1,i\neq t}^T (\bar{R}_{i,i}+1)$.
Furthermore, it is easy to see that the constant 1 is the only
constant term in $C_{t,t}$. Thus, $C_{t,t}$ can be rewritten as
$C_{t,t} = \bar{C}_{t,t}+1$, where no constant term exists in
$\bar{C}_{t,t}$. Consequently, $[\bmR^{-1}]_{t,t}$ can be
rewritten as $[\bmR^{-1}]_{t,t} = \bar{C}_{t,t}/\mathrm{det}(\bmR)
+ 1/\mathrm{det}(\bmR)$. When $t_1 \neq t_2$, $C_{t_2,t_1}$ does
not contain any constant term, and hence, $[\bmR^{-1}]_{t_1,t_2}$
does not contain the term
$1/\mathrm{det}(\bmR)$.\footnote{$C_{t_2,t_1}$ may be zero, but it
does not change the conclusion that $[\bmR^{-1}]_{t_1,t_2}$ does
not contain the term $1/\mathrm{det}(\bmR)$.} Therefore, we can
extract the term $1/\mathrm{det}(\bmR)$ from every main diagonal
entry of $\bmR^{-1}$ and rewrite $\bmR^{-1}$ in the following way
\begin{eqnarray}\label{eqn:RinvI}
\bmR^{-1}
&=&\frac{1}{\mathrm{det}(\bmR)}\overline{\bmR}+\frac{1}{\mathrm{det}(\bmR)}\bmI.
\end{eqnarray}
Substituting (\ref{eqn:RinvI}) into (\ref{eqn:orth}) gives us
\begin{eqnarray}
\bmX_D\bmR^{-1}\bmX_D^H &=&
\frac{1}{\mathrm{det}(\bmR)}\left(\bmX_D\overline{\bmR}\bmX_D^H+\bmX_D\bmX_D^H\right)\\
&=&|s_1|^2\bmD_1+\cdots+|s_N|^2\bmD_N.\label{eqn:xrxxx}
\end{eqnarray}
Note that $\overline{\bmR}$ is a random matrix and it does not
contain any constant terms. In order to make (\ref{eqn:xrxxx})
hold for every possible $\overline{\bmR}$, $\bmX_D\bmX_D^H$ must
be diagonal and it can be denoted by (\ref{eqn:orthE}).


Secondly, we show that $E_{n,k}$ is strictly positive. From
(\ref{eqn:orth}) and (\ref{eqn:orthE}), we have
\begin{eqnarray}
D_{n,k} &=& \sum_{t=1}^T \sum_{i=1}^T [\bmR^{-1}]_{i,t}
([\bmA_k]_{n,i} [\bmA_k]_{n,t}^* + [\bmB_k]_{n,i}^*
[\bmB_k]_{n,t})\\\label{eqn:ARABRAelement2}
 E_{n,k} &=& \sum_{t=1}^T(|[\bmA_k]_{n,t}|^2
+ |[\bmB_k]_{n,t}|^2).\label{eqn:AABBelement2}
\end{eqnarray}
Since $D_{n,k}$ is non-zero, at least one $[\bmA_k]_{n,t}$ or one
$[\bmB_k]_{n,t}$ is non-zero. Therefore,
$E_{n,k}=\sum_{t=1}^T(|[\bmA_k]_{n,t}|^2 + |[\bmB_k]_{n,t}|^2)$ is
strictly positive.


Lastly, we prove (\ref{eqn:Econd1})--(\ref{eqn:Econd5}). When
$k_1\neq k_2$, it follows from (\ref{eqn:orthE}) that
$[\bmX_D\bmR^{-1}\bmX_D]_{k_1,k_2}$ is given by
\begin{eqnarray}
[\bmX_D\bmX_D^H]_{k_1,k_2}
&=&h_{k_1}h_{k_2}^{*}\bms\bmA_{k_1}\bmA_{k_2}^H\bms^H+
h_{k_1}^*h_{k_2}^{*}\bms^*\bmB_{k_1}\bmA_{k_2}^H\bms^H\nonumber\\
&&+h_{k_1}h_{k_2}\bms\bmA_{k_1}\bmB_{k_2}^H\bms^T+
h_{k_1}^*h_{k_2}\bms^*\bmB_{k_1}\bmB_{k_2}^H\bms^T\nonumber\\ %%\label{eqn:sum1}\\
&=&0.\label{eqn:sum2}
\end{eqnarray}
Note that $h_{k_1}$ and $h_{k_2}$ can be any complex numbers.
Thus, in order to make (\ref{eqn:sum2}) hold for every possible
value of $h_{k_1}$ and $h_{k_2}$, the following equalities must
hold
\begin{eqnarray}
\bms\bmA_{k_1}\bmA_{k_2}^H\bms^H=\bms^*\bmB_{k_1}\bmB_{k_2}^H\bms^T=0.
\end{eqnarray}
By using Lemma 1 of \cite{liang2}, we have (\ref{eqn:Econd1}) and
(\ref{eqn:Econd2}). When $k_1=k_2=k$, by (\ref{eqn:orthE}),
$[\bmX_D\bmX_D^H]_{k,k}$ is given by
\begin{eqnarray}
[\bmX_D\bmX_D^H]_{k,k} &=&|h_{k}|^2\bms(\bmA_{k}\bmA_{k}^H+
\bmB_{k}^*\bmB_{k}^T)\bms^H\nonumber\\
&&+h_{k}^*h_{k}^{*}\bms^*\bmB_{k}\bmA_{k}^H\bms^H
+h_{k}h_{k}\bms\bmA_{k_1}\bmB_{k}^H\bms^T\nonumber\\
&=&|h_k|^2\bms \ {\mathrm{diag}}[E_{1,k},\cdots,E_{N,k}]\bms^H.
\end{eqnarray}
For the same reason as in (\ref{eqn:sum2}), the following equality
must hold
\begin{eqnarray}
\bms(\bmA_{k}\bmA_{k}^H+ \bmB_{k}^*\bmB_{k}^T)\bms^H &=&\bms \
{\mathrm{diag}}[E_{1,k},\cdots,E_{N,k}]\bms^H.
\end{eqnarray}
By using Lemma 1 of \cite{liang2} again, we have
(\ref{eqn:Econd5}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendices
%\vspace{1cm}
\section*{Appendix D}
\renewcommand\theequation{D.\arabic{equation}}
\setcounter{equation}{0}

We first prove (\ref{eqn:CSIcond1})--(\ref{eqn:CSIcond3}). By
(\ref{eqn:orthF}), we can write $F_{n,k}$ as $F_{n,k}=\sum_{i=1}^K
F_{n,k}^{f_i} |\rho f_i|^2 + F_{n,k}^{0}$, where $F_{n,k}^{0}$ and
$F_{n,k}^{f_i}$ are just constants. Furthermore, we notice that
$E_{n,k}$ does not have any terms containing $|\rho f_k|^2$ by
(\ref{eqn:orthEcsi}).


The value of $[\bmX_C(\bmR-\bmI)\bmX^H]_{k,k}$ can be obtained by
(\ref{eqn:orthEcsi}) and (\ref{eqn:orthF})
\begin{eqnarray}
[\bmX_C(\bmR-\bmI)\bmX_C^H]_{k,k}
&=&\bms\bmA_{k}(\bmR-\bmI)\bmA_{k}^H\bms^H+
\bms^*\bmB_{k}(\bmR-\bmI)\bmA_{k}^H\bms^H\nonumber\\
&&+\bms\bmA_{k}(\bmR-\bmI)\bmB_{k}^H\bms^T+
\bms^*\bmB_{k}(\bmR-\bmI)\bmB_{k}^H\bms^T\nonumber\\
&=&\bms \ {\mathrm{diag}}[F_{1,k}-E_{1,k},\cdots,F_{N,k}-E_{N,k}]\
\bms^H.
\end{eqnarray}
By using Lemma 1 of \cite{liang2}, we have
\begin{eqnarray}
\bmA_{k}(\bmR-\bmI)\bmA_{k}^H + \bmB_{k}^*(\bmR-\bmI)\bmB_{k}^T
&=&
{\mathrm{diag}}[F_{1,k}-E_{1,k},\cdots,F_{N,k}-E_{1,k}]\label{eqn:a1a1b1b1}\\
\bmA_{k} (\bmR-\bmI) \bmB_{k}^H + \bmB_{k}^{*}(\bmR-\bmI)
\bmA_{k}^T &=& \bmzero\label{eqn:abkk}\\
\bmB_{k}(\bmR-\bmI)\bmA_{k}^H + \bmA_{k}^*(\bmR-\bmI)\bmB_{k}^T
&=& \bmzero.\label{eqn:bakk}
\end{eqnarray}
The matrix $\bmR-\bmI$ can be obtained form (\ref{eqn:R}) and
substituting it into (\ref{eqn:a1a1b1b1}) gives us
\begin{eqnarray}\label{eqn:suma1a1b1b1}
&&\sum_{i=1}^K |\rho f_k|^2 \left(\bmA_{k}(\bmA_i^H\bmA_i
+\bmB_i^H\bmB_i)\bmA_{k}^H + \bmB_{k}^*(\bmA_i^H\bmA_i
+\bmB_i^H\bmB_i)\bmB_{k}^T\right) \\
&=& {\mathrm{diag}}[F_{1,k}-E_{1,k},\cdots,F_{N,k}-E_{N,k}].
\end{eqnarray}
Note that $f_i$ can be any complex numbers. Thus, in order to make
(\ref{eqn:suma1a1b1b1}) hold for every possible $f_i$, we must
have (\ref{eqn:CSIcond1}). Similarly, (\ref{eqn:abkk}) and
(\ref{eqn:bakk}) implies
\begin{eqnarray}
\bmA_{k} (\bmA_i^H\bmA_i +\bmB_i^H\bmB_i) \bmB_{k}^H +
\bmB_{k}^{*}(\bmA_i^H\bmA_i +\bmB_i^H\bmB_i)
\bmA_{k}^T &=& \bmzero, \label{eqn:abkkaabb}\\
\bmB_{k}(\bmA_k^H\bmA_i +\bmB_k^H\bmB_i)\bmA_{k}^H +
\bmA_{k}^*(\bmA_k^H\bmA_i +\bmB_k^H\bmB_i)\bmB_{k}^T &=&
\bmzero.\label{eqn:bakkaabb}
\end{eqnarray}

When $k_1\neq k_2$, the value of
$[\bmX_C(\bmR-\bmI)\bmX_C^H]_{k_1,k_2}$ is given by
\begin{eqnarray}
[\bmX_C(\bmR-\bmI)\bmX_C^H]_{k_1,k_2}
&=&\bms\bmA_{k_1}(\bmR-\bmI)\bmA_{k_2}^H\bms^H+
\bms^*\bmB_{k_1}(\bmR-\bmI)\bmA_{k_2}^H\bms^H\nonumber\\
&&+\bms\bmA_{k_1}(\bmR-\bmI)\bmB_{k_2}^H\bms^T+
\bms^*\bmB_{k_1}(\bmR-\bmI)\bmB_{k_2}^H\bms^T\nonumber\\
&=&0.
\end{eqnarray}
By using Lemma 1 of \cite{liang2} and noting that $f_k$ can be any
complex numbers, we must have (\ref{eqn:CSIcond1}) and the
following two equalities
\begin{eqnarray}
\bmA_{k_1} (\bmA_k^H\bmA_k +\bmB_k^H\bmB_k) \bmB_{k_2}^H +
\bmB_{k_2}^{*}(\bmA_k^H\bmA_k +\bmB_k^H\bmB_k)
\bmA_{k_1}^T &=& \bmzero, \ \ \ k_1\neq k_2\label{eqn:abk1k2}\\
\bmB_{k_1}(\bmA_k^H\bmA_k +\bmB_k^H\bmB_k)\bmA_{k_2}^H +
\bmA_{k_2}^*(\bmA_k^H\bmA_k +\bmB_k^H\bmB_k)\bmB_{k_1}^T &=&
\bmzero, \ \ \ k_1\neq k_2.\label{eqn:bak1k2}
\end{eqnarray}
Based on (\ref{eqn:abkkaabb}), (\ref{eqn:abk1k2}),
(\ref{eqn:bakkaabb}), and (\ref{eqn:bak1k2}), it is immediate to
obtain (\ref{eqn:CSIcond2}) and (\ref{eqn:CSIcond3}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Secondly, when $w\geq 3$, we show that the data-rate $N_w/T_w$ of
$\tilde{\bmX}_{Cw}$ is exactly $1/2$. Theorem \ref{thm:partition}
tells us $\tilde{\bmX}_{Cw}$ are row-monomial DOSTBCs-CPI, and
hence, the associated matrices $\tilde{\bmA}^w_k$ and
$\tilde{\bmB}^w_k$ satisfy the row-monomial condition.
Furthermore, as we have seen in Appendix F, every entry in
$\tilde{\bmX}_{Cw}$ is non-zero. Therefore, it is not hard to see
that $T_w={\mathrm{rank}}([\tilde{\bmA}^w_k;\tilde{\bmB}^w_k])$,
for $1\leq k\leq K_w$. By using the uniform transform proposed in
\cite{wang}, we can write $\tilde{\bmA}^w_k$ and
$\tilde{\bmB}^w_k$ as follows: when $k=1$,
\begin{eqnarray}
\tilde{\bmA}^w_1 =\left(%
\begin{array}{cccc}
  \bmD_{\lambda} &\bmzero & \bmzero  \\
  \bmzero & \bmI & \bmzero \\
\end{array}%
\right)&&
\tilde{\bmB}^w_1 =\left(%
\begin{array}{cccc}
  \bmzero & \bmzero & \bmD_{\mu}  \\
  \bmzero & \bmzero & \bmzero
\end{array}%
\right);
\end{eqnarray}
when $1<k\leq K_w$,
\begin{eqnarray}\label{eqn:akbkzero}
\tilde{\bmA}^w_k =\left(%
\begin{array}{cccc}
  \tilde{\bmA}^w_{k1} & \tilde{\bmA}^w_{k3} & \tilde{\bmA}^w_{k5}  \\
  \bmzero & \bmzero & \bmzero \\
\end{array}%
\right)&&
\tilde{\bmB}^w_k =\left(%
\begin{array}{cccc}
  \tilde{\bmB}^w_{k1} & \tilde{\bmB}^w_{k3} & \tilde{\bmB}^w_{k5}  \\
  \tilde{\bmB}^w_{k2} & \tilde{\bmB}^w_{k4} & \tilde{\bmB}^w_{k6} \\
\end{array}%
\right).
\end{eqnarray}
The dimensions of the sub-matrices have been described in detail
in \cite{wang}, and hence, we do not repeat them here. Moreover,
like in \cite{wang}, note that the uniform transform does not
change the properties of $\tilde{\bmA}^w_k$ and
$\tilde{\bmB}^w_k$, which can be shown by tedious but
straightforward calculation.


Because $\tilde{\bmX}_{Cw}$ is a row-monomial DOSTBC-CPI,
$\tilde{\bmA}^w_k$ and $\tilde{\bmB}^w_k$ satisfy all the
conditions (\ref{eqn:aabb})--(\ref{eqn:baab}) and
(\ref{eqn:CSIcond1})--(\ref{eqn:CSIcond3}). It follows from
(\ref{eqn:aabb}) that
$\tilde{\bmA}_{1}^w\tilde{\bmA}_{k}^{wH}+\tilde{\bmB}_{k}^{w*}\tilde{\bmB}_{1}^{wT}=0$
that
$\tilde{\bmA}_{k3}^H+\tilde{\bmB}_{k6}^*\bmD_{\lambda}=\bmzero$
for $k\neq 1$. On the other hand, by (\ref{eqn:CSIcond1}),
$\tilde{\bmA}_{1}^w(\tilde{\bmA}_1^{wH}\tilde{\bmA}_1^w
+\tilde{\bmB}_1^{wH}\tilde{\bmB}_1^w)\tilde{\bmA}_{k}^{wH}+\tilde{\bmB}_{k}^{w*}(\tilde{\bmA}_1^{wH}\tilde{\bmA}_1^w
+\tilde{\bmB}_1^{wH}\tilde{\bmB}_1^w)\tilde{\bmB}_{1}^{wT}=0$ for
$k\neq 1$ and it implies
$\tilde{\bmA}_{k3}^{wH}+\tilde{\bmB}_{k6}^{w*}\bmD_{\lambda}\bmD_{\lambda}\bmD_{\lambda}=\bmzero$.
Thus,
$\tilde{\bmB}_{k6}^{w*}\bmD_{\lambda}\bmD_{\lambda}\bmD_{\lambda}=\tilde{\bmB}_{k6}^{w*}\bmD_{\lambda}$.
It has been shown that $\bmD_{\lambda}$ is diagonal and its main
diagonal entries are strictly less than $1$. Thus, it is not hard
to see that $\tilde{\bmB}_{k6}=\bmzero$ for $k\neq 1$.
Furthermore, by (\ref{eqn:abba}),
$\tilde{\bmA}_1^w\tilde{\bmB}_k^{wH}+\tilde{\bmB}_k^{w*}\tilde{\bmA}_1^{wT}=\bmzero$
and it implies
$\bmD_{\lambda}\tilde{\bmB}_{k2}^{wH}+\tilde{\bmB}_{k3}^{w*}=\bmzero$.
On the other hand, by (\ref{eqn:CSIcond2}),
$\tilde{\bmA}_1^w(\tilde{\bmA}_1^{wH}\tilde{\bmA}_1
+\tilde{\bmB}_1^{wH}\tilde{\bmB}_1^w)\tilde{\bmB}_k^{wH}+\tilde{\bmB}_k^{w*}(\tilde{\bmA}_1^{wH}\tilde{\bmA}_1^w
+\tilde{\bmB}_1^{wH}\tilde{\bmB}_1^w)\tilde{\bmA}_1^{wT}=\bmzero$
and it implies
$\bmD_{\lambda}\bmD_{\lambda}\bmD_{\lambda}\tilde{\bmB}_{k2}^H+\tilde{\bmB}_{k3}^*=\bmzero$.
Like $\bmD_{\lambda}$, $\bmD_{\mu}$ is also diagonal and its main
diagonal entries are strictly less than $1$ \cite{wang}. Thus, it
is not hard to get $\tilde{\bmB}_{k2}=\bmzero$ for $k\neq 1$.

Then, we focus on the matrix $\tilde{\bmB}^w_{k4}$, whose
dimension is $(2N_w-T_w)\times(N_w-T_w)$. Because
$\tilde{\bmA}_k^w$ and $\tilde{\bmB}_k^w$ satisfy
(\ref{eqn:aabb}), we notice that
$\tilde{\bmB}_{k_24}^{w*}\tilde{\bmB}_{k_14}^{wT}=\bmzero$, when
$k_1\neq k_2$ and they are both larger than one. When
$1<k_1=k_2=k\leq K_w$, (\ref{eqn:aabb}) suggests that
$\tilde{\bmA}_{k}^w\tilde{\bmA}_{k}^{wH}+\tilde{\bmB}_{k}^{w*}\tilde{\bmB}_{k}^{wT}$
has full rank and it implies that
$\tilde{\bmB}_{k4}^{w*}\tilde{\bmB}_{k4}^{wT}$ has full rank.
Therefore, the $(2N_w-T_w)(K_w-1)$ rows in the matrix
$[\tilde{\bmB}^w_{24};\tilde{\bmB}^w_{34};\cdots;\tilde{\bmB}^w_{K_w4}]$
are linearly independent and this leads to $(2N_w-T_w)(K_w-1)\leq
2N_w-T_w$. When $K_w>2$, we get $2N_w-T_w\leq0$, and hence,
$2N_w\leq T_w$. On the other hand, because
$T_w={\mathrm{rank}}[\tilde{\bmA}^w_1;\tilde{\bmB}^w_1]$ and the
dimension of $[\tilde{\bmA}^w_1;\tilde{\bmB}^w_1]$ is $2N_w\times
T_w$, we have $T_w\leq 2N_w$. Therefore, $T_w=2N_w$ and the
data-rate $N_w/T_w$ of $\tilde{\bmX}_{Cw}$ is exactly $1/2$ when
$K_w>2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\appendices
%\vspace{1cm}
\section*{Appendix C}
\renewcommand\theequation{C.\arabic{equation}}
\setcounter{equation}{0}

For convenience, we refer to the product $\prod_{k=1}^K |\rho
f_k|^{2t_k}$ with $\sum_{k=1}^Kt_k = t$ as the $t$-th order term
of $|\rho f_k|^{2}$. We first expand $\bmR^{-1}$ as follows:
\begin{equation}
\bmR^{-1} =
\frac{1}{{\mathrm{det}}(\bmR)}\left(\bmR^0+\bmR^1+\cdots+\bmR^{T-1}\right),
\end{equation}
The entries in $\bmR^t$ are either zero or the $t$-th order term
of $|\rho f_k|^{2}$. Because $\bmX_C\bmR^{-1}\bmX_C^H$ is denoted
by (\ref{eqn:orthcsi}) and $f_k$ can be any value, it is not hard
to see that $\bmX_C\bmR^t\bmX_C^H$ can be denoted as follows:
\begin{equation}\label{eqn:XRtX}
\bmX_C\bmR^t\bmX_C^H = |s_1|^2\bmH^t_1 + \cdots+ |s_N|^2\bmH^t_N,
\end{equation}
where $\bmH_n^t$ is diagonal. For example, Theorem
\ref{thm:necessary} suggests that $\bmR^0 = \bmI$ and
$\bmH^0_n=\bmE_n$.

We are particularly interested on the structure of $\bmR^1$ whose
entries can only be zero or $|\rho f_k|^{2}$. As shown in Appendix
A, we can write $[\bmR]_{t,t}$ as $[\bmR]_{t,t}=\bar{R}_{t,t}+1$.
$[\bmR^{-1}]_{t_1,t_2}$ is given by $[\bmR^{-1}]_{t_1,t_2} =
C_{t_2,t_1}/\mathrm{det}(\bmR)$, where $C_{t_2,t_1}$ is the matrix
cofactor of $[\bmR]_{t_2,t_1}$. $C_{t_2,t_1}$ is given by
$C_{t_2,t_1}=(-1)^{t_2+t_1} {\mathrm{det}}(\bmM_{t_2,t_1})$, where
$\bmM_{t_2,t_1}$ is obtained by deleting the $t_2$-th row and the
$t_1$-th column from $\bmR$. When $t_1 =t_2=t$, $C_{t,t}$ contains
the summation $\sum_{i=1,i\neq t}^T\bar{R}_{i,i}$ and it is
generated by $\prod_{i=1,i\neq t}^T [\bmR]_{i,i} =
\prod_{i=1,i\neq t}^T (\bar{R}_{i,i}+1)$, which is the product of
the main diagonal entries of $\bmM_{t,t}$. Because $\bar{R}_{i,i}$
is a summation of several first order terms of $|\rho f_k|^2$,
$\sum_{i=1,i\neq t}^T\bar{R}_{i,i}$ is also a summation of many
first order terms of $|\rho f_k|^2$, and hence, it is a part of
$[\bmR^1]_{t,t}$. Furthermore, we notice that only the product of
the main diagonal entries in $\bmM_{t,t}$ can generate the first
order terms of $|\rho f_k|^2$. Therefore, we have $[\bmR^1]_{t,t}
=\sum_{i=1,i\neq t}^T\bar{R}_{i,i}$.

When $t_1\neq t_2$, it is not hard to show that $C_{t_2,t_1}$
contains only one first order term of $|\rho f_k|$, which is just
$-[\bmR]_{t_1,t_2}$. Precise proof can be easily done by using
mathematical induction on the dimension of $\bmR$. Therefore, we
conclude that the main diagonal entries of $\bmR^1$ are given by
$[\bmR^1]_{t,t}=\sum_{i=1,i\neq t}^T\bar{R}_{i,i}$ and the
off-diagonal entries are given by
$[\bmR^1]_{t_1,t_2}=-[\bmR]_{t_1,t_2}$. Furthermore, by
(\ref{eqn:orthEcsi}) and (\ref{eqn:XRtX}), the matrix $\bmX_C \bmR
\bmX_C^H={\mathrm{Tr}}(\bmR)\bmX_C\bmX_C^H - \bmX_C \bmR^1
\bmX_C^H$ can be denoted by (\ref{eqn:orthF}) and $\bmF_n =
{\mathrm{Tr}}(\bmR) \bmE_n - \bmH_n^1$ is diagonal.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{wang} H. Wang and X.-G. Xia, ``Upper bounds of rates of complex orthogonal
space-time block codes,'' {\it IEEE Trans. Inform. Theory,} vol.
49. pp. 2788--2796, Oct. 2003.

\bibitem{liang2} X.-B. Liang and X.-G. Xia, ``On the nonexistence
of rate-one generalized complex orthogonal designs,'' {\it IEEE
Trans. Inform. Theory,} vol. 49, pp. 2984--2989, Nov. 2003.

\bibitem{su1} W. Su and X.-G. Xia, ``Two generalized complex orthogonal space-time
block codes of rates 7/11 and 3/5 for 5 and 6 transmit antennas,''
{\it IEEE Trans. Inform. Theory}, vol. 49, pp. 313--316, Jan.
2003.

\bibitem{su2} W. Su, X.-G. Xia, and K. J. R. Liu, ``A systematic design of high-rate
complex orthogonal space-time block codes,'' {\it IEEE Commun.
Lett.}, vol. 8, pp. 380--382, June 2004.

\bibitem{shen} H.-B. Kan and H. Shen, ``A counterexample for the open problem on the
minimal delays of orthogonal designs with maximal rates,'' {\it
IEEE Trans. Inform. Theory}, vol. 51, pp. 355--359, Jan. 2005.


\bibitem{liang1} X.-B. Liang, ``Orthogonal designs with
maximal rates,'' \emph{IEEE Trans. Inform. Theory}, vol. 49, pp.
2468--2503, Oct. 2003.

